BRS symmetry restoration of chiral Abelian Higgs-Kibble theory in dimensional renormalization with a non-anticommuting $\gamma_5$

The one-loop renormalization of the abelian Higgs-Kibble model in a general 't Hooft gauge and with chiral fermions is fully worked out within dimensional renormalization scheme with a non-anticommuting $\gamma_5$. The anomalous terms introduced in the Slavnov-Taylor identities by the minimal subtraction algorithm are calculated and the asymmetric counterterms needed to restore the BRS symmetry, if the anomaly cancellation conditions are met, are computed. The computations draw heavily from regularized action principles and Algebraic Renormalization theory.

==> Article/functions <==
__totex(){
echo  > "$2"
echo '\def\frac#1#2{{\displaystyle #1}\over{\displaystyle #2}}' >> "$2"
echo '\def\frac#1#2{{\displaystyle #1}\over{\displaystyle #2}}' >> "$2"
cat "$1" |\
   tr "\012" "ç" | sed 's/ç/ ç /g' |\
   sed -e 's/\\Mvariable//g' \
       -e 's/\\Muserfunction//g' \
       -e 's/\\gamma\\\\_{5}/\\gamma_5/g'  \
       -e 's/\\_/\^/g'  \
       -e 's/mu1/\\mu_1/g'  \
       -e 's/mu2/\\mu_2/g'  \
       -e 's/mu3/\\mu_3/g'  \
       -e 's/mu4/\\mu_4/g'  \
       -e 's/k1/k_1/g'  \
       -e 's/k2/k_2/g'  \
       -e 's/k3/k_3/g'  \
       -e 's/k4/k_4/g'  \
       -e 's/\\phi1/{\\phi_1}/g'  \
       -e 's/\\phi2/{\\phi_2}/g'  \
       -e 's/\\phi3/{\\phi_3}/g'  \
       -e 's/\\phi4/{\\phi_4}/g'  \
       -e 's/cteI//g'  \
       -e 's/cte4//g'  \
       -e 's/type/r/g'  \
       -e 's/theta/\\theta/g'  \
       -e 's/lambda/\\lambda/g'  \
       -e 's/\\,1/\\un/g'  \
       -e 's/\\frac{-{}}/\\frac{-{1}}/g'  \
       -e 's/\\frac{{}}/\\frac{{1}}/g'  \
       -e 's/{xi1}/{\\xi^\\prime}/g'  \
       -e 's/rho/\\rho/g'  \
       -e 's/{{gg}}\^2/g\^2/g'  \
       -e 's/\\RawWedge  */\^/g' \
       -e 's/-[ ç]*{\\frac/\\cr \& - {\\frac/g'  \
       -e 's/+[ ç]*{\\frac/\\cr \& + {\\frac/g'  |\
     tr "ç" "\012"  >> "$2"
echo  >> "$2"
}
     
__tops(){
 filename=`echo "$1" | cut -f1 -d'.'`
 tex $1 && dvips -o "$filename".ps -D600 "$filename".dvi
}

__tomatrix(){
echo '\def\frac#1#2{{#1}\over{#2}}' > "$2"
cat "$1" |\
   sed -e 's/\\Mvariable//g' \
       -e 's/\\Muserfunction//g' \
       -e 's/\\gamma\\\\_{5}/\\gamma_5/g'  \
       -e 's/\\_/\^/g'  \
       -e 's/\\\&/\&/g'  \
       -e 's/\\matrix/\\left(\\matrix/' \
       -e 's/\\cr *}/\\cr }\\right)/' \
       -e 's/mumu/\\mu\^2/g'  \
       -e 's/cteI//g'  \
       -e 's/type/r/g'  \
       -e 's/theta/\\theta/g'  \
       -e 's/lambda/\\lambda/g'  \
       -e 's/{xi1}/{\\xi^\\prime}/g'  \
       -e 's/rho/\\rho/g'  \
       -e 's/{{gg}}\^2/g\^2/g'  \
       -e 's/\\RawWedge  */\^/g' >> "$2"
echo  >> "$2"
}
     
__tops(){
 filename=`echo "$1" | cut -f1 -d'.'`
 tex $1 && dvips -o "$filename".ps -D600 "$filename".dvi
}


==> README <==
%auto-ignore 
====================================================================
Mathematica programs and TeX source needed to reproduce 
and generate the paper:
"BRS symmetry restoration of chiral Abelian Higgs-Kibble theory
in dimensional renormalization with a non-anticommuting $\gamma_5$",
by Domingo Sanchez-Ruiz <domingo@toboso.fis.ucm.es>
====================================================================
September 2002

* TeX source is plain tex, and the main file is 'bmqah.tex', so do
"tex bmqah.tex" to generate the paper

* The macro epsf, not included in this distribution but
avalaible in http://arXiv.org/ftp/macros/,
all *.tex files under the Article subdirectory 
and all *.eps files under the Images subdirectory
are needed in order to 'tex' the file bmqah.tex

* To redo all the Mathematica computations and regenerate
the TeX source of the tex files with the results, do in
a sh-like shell:
chmod +x *.sh
chmod +x Programs/*.sh
chmod +x Article/*.sh
 (or any other command to make executable
the shell scripts )
./batch-all.sh

You will need Mathematica 3.0 (maybe the programs work with
later versions) and its command line interface, named 'math',
in the shell path. 

NOTE 1: in a 2.2 Linux box on Pentium II - 300 Mhz with
Mathematica 3.0 it takes about seven hours. Sorry, we had
no much time, and we prefer to do general programs rather
than fast programs. And they are not meant to be very valuable
programs, we incorporate them mainly because we think they are very
important for a conscientious revision and reproduction of the results.
All steps of a investigation should be public.

NOTE 2: You can redistribute our programs and/or modify it under the
   terms of the GNU General Public License as published by
   the Free Software Foundation; either version 2 of the License
   (see file Programs/COPYING), or any later version. 
 
(C) 2000,2002, Domingo Sanchez-Ruiz <domingo@toboso.fis.ucm.es>

